Saturation-Aware Space-Variant Blind Image Deblurring

This paper presents a novel saturation aware space variant blind image deblurring framework designed to address challenges posed by saturated pixels in deblurring under high dynamic range and low light conditions. The proposed approach effectively segments the image based on blur intensity and proximity to saturation, leveraging a pre estimated Light Spread Function to mitigate stray light effects. By accurately estimating the true radiance of saturated regions using the dark channel prior, our method enhances the deblurring process without introducing artifacts like ringing. Experimental evaluations on both synthetic and real world datasets demonstrate that the framework improves deblurring outcomes across various scenarios showcasing superior performance compared to state of the art saturation-aware and general purpose methods. This adaptability highlights the framework potential integration with existing and emerging blind image deblurring techniques.

==> sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.
% \begin{figure*}[!h]
% \centering
% \begin{subfigure}{1.3in}
% {\includegraphics[width=1.3in,height=1.3in,keepaspectratio]{sec/images/Dark1.png}}
%  \caption{Seahorse}
% \end{subfigure}\hfill
% \begin{subfigure}{1.3in}
% {\includegraphics[width=1.3in,height=1.3in,keepaspectratio]{sec/images/5 dark.png}}
%  \caption{Seahorse}
% \end{subfigure}\hfill
% \begin{subfigure}{1.3in}
% {\includegraphics[width=1.3in,height=1.3in,keepaspectratio]{sec/images/15 dark.png}}
%  \caption{Seahorse}
% \end{subfigure}\hfill
% \begin{subfigure}{1.3in}
% {\includegraphics[width=1.3in,height=1.3in,keepaspectratio]{sec/images/15 dark.png}}
%  \caption{Seahorse}
% \end{subfigure}\\
% \begin{subfigure}{1.3in}
% {\includegraphics[width=1.3in,height=1.3in,keepaspectratio]{sec/images/1 dark_im.png}}
%  \caption{Seahorse}
% \end{subfigure}\hfill
% \begin{subfigure}{1.3in}
% {\includegraphics[width=1.3in,height=1.3in,keepaspectratio]{sec/images/2 dark_im.png}}
%  \caption{Seahorse}
% \end{subfigure}\hfill
% \begin{subfigure}{1.3in}
% {\includegraphics[width=1.3in,height=1.3in,keepaspectratio]{sec/images/3 dark_im.png}}
%  \caption{Seahorse}
% \end{subfigure}\hfill
% \begin{subfigure}{1.3in}
% {\includegraphics[width=1.3in,height=1.3in,keepaspectratio]{sec/images/4 dark_im.png}}
%  \caption{Seahorse}
% \end{subfigure}\hfill\\
%  \caption{Seahorse}
%  \end{figure*}
%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/Experimental_results.tex <==



\section{Final copy}
In this section, we provide the quantitave and qualitative comparsion of the prosed method with the state of the art image deblurring techniques desinged specificaly for saturation handling as well as more general methods. We tested our algorithm on both synthetics and real dataset in our comparsions to demonstrate the robustness of the proposed method. Our method is implemented in MATLAB  on a computer with an RTX 4070 GPU and 32.0 GB RAM. The propsed deblurring framework, works in two phases where saturation estimation happens in the first stage and then them image with predicted saturated regions is deblureed exisitng. In all of our esperiments we have used \cite{xu2010two}, as the prime blind image debluuring method, additionaly we have tried some other exisitng debluuring techniques to ensure that the proosed framework can be adopted with latest space varitned blind image deblurring techniques in the future to reap the bebenfits of latest reserch in image deblurring.\\
To effectively examine the robustness of the proposed method under varying level of brightness, we adopted the dataset \cite{hanji2021hdr4cv}, as it provides a stack of varying expousre image. Specificaly we adopted the tunnel scene becuase it exhibit a high dynamic range as shown in Figure \ref{expourse view}. The dataset provides a sequence of 100 images of static scene with contorlled camera motion, For the results presented in Figure \ref{Varying exposure}, the blurring imnput image is generted by merging five consecutive frames in the sequence. In the experiment we demonstrate the how different satuatre awaere deblurring methods compare agaisnt the propsed methods under verying expourse ondition. It can been seen that propsed methods performs moderatley in comparsion with other methods for the low expourse image, however its perfomance peeks in comparion to other methods as the saturation in the input image increase, showing it effectivens against images with saturation. For non-blind image deblurring techniques that handels saturation \cite{}, the blur kernel is estimated using the best performing method in the comparison.
\begin{figure*}[!h]
\centering
\begin{subfigure}{1.3in}
{\includegraphics[width=1.3in,height=1.3in,keepaspectratio]{sec/images/exp_1.png}}
 \caption{Seahorse}
\end{subfigure}\hfill
\begin{subfigure}{1.3in}
{\includegraphics[width=1.3in,height=1.3in,keepaspectratio]{sec/images/exp_2.png}}
 \caption{Seahorse}
\end{subfigure}\hfill
\begin{subfigure}{1.3in}
{\includegraphics[width=1.3in,height=1.3in,keepaspectratio]{sec/images/exp_3.png}}
 \caption{Seahorse}
\end{subfigure}\hfill
\begin{subfigure}{1.3in}
{\includegraphics[width=1.3in,height=1.3in,keepaspectratio]{sec/images/exp_4.png}}
 \caption{Seahorse}
\end{subfigure}\hfill
\begin{subfigure}{1.3in}
{\includegraphics[width=1.3in,height=1.3in,keepaspectratio]{sec/images/exp_5.png}}
 \caption{Seahorse}
\end{subfigure}\hfill\\
 \label{expourse view}
 \caption{A stack of varying exposure frames for a single images from the tunnel scene of \cite{hanji2021hdr4cv}, used to generate the results in \ref{varying exposure}}
 \end{figure*}
 
\begin{figure}[!h]
\centering
{\includegraphics[trim={45 7 30 23},clip,width=3.5in,height=3.5in,keepaspectratio]{sec/images/Varying exposure_result.pdf}}
\label{Varying exposure}
 \caption{Compsrision of the propsed method with the exisitng image deblurring methods designed specificaly for saturation handling in image deblurring.}
\end{figure}\\

We demonstrante the sucess of the propsed method on a dataset captured in real environment \cite{nah2017deep}. Specifically we seleted test sequence $"GOPR0881_11_01"$ which provide siginficant saturated regions in every image of the sequence and has signifact dynamic range to offer. In this experiment we used the proposed framework with an additional image deblurring technique \cite{wen2020simple} to show that the proposed framework does not derive it strgent from a pirticualr deblurring algorithm  and any SVBID algorithm could benefit from the propoed framework when dealing with saturated images. Again for the comprsion methods that are non-blind the kernels from the best performing method are used. Figure \ref{real_dataset} shows that the proped framework with two different deblurring methods surpass 
 both qualitatively and quantaively  the state of the art methods saturation aware deblurring methods.
%  \begin{figure*}[h]
% \centering
% \vspace{0.0in}
% % \raisebox{.8\height}{ \rotatebox[origin=]{90}{Proposed}}
%  \begin{subfigure}{2.0in}
%  \begin{tikzpicture}
%    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=2.0in,height=2.0in,keepaspectratio]{sec/images/prop_data2.png}};
%     \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[red,ultra thick,sharp corners] (0.07,0.65) rectangle (0.13,0.57);
%     \end{scope}
%      \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[blue,ultra thick,sharp corners] (0.35,0.57) rectangle (0.39,0.53);
%     \end{scope}
% \end{tikzpicture}
%  % \caption{PSNR = 25.00, SSIM = 0.89}}
%   \end{subfigure}\\
%   \hspace{-0.07in}
%   \begin{subfigure}{0.96in}
%   \setlength{\fboxsep}{0pt}
% \adjustbox{cfbox=red 1pt}{\includegraphics[trim={45 210 565 134},clip,width=0.96in,height=0.96in,keepaspectratio]{sec/images/prop_data2.png}}
%   \end{subfigure}
%   \begin{subfigure}{0.975in}
%   \setlength{\fboxsep}{0pt}
% \adjustbox{cfbox=blue 1pt}{\includegraphics[width=2cm,trim={ 226 190 393 159},clip,width=0.975in,height=0.975in,keepaspectratio]{sec/images/prop_data2.png}}  \end{subfigure}\hfill\\
% % \raisebox{.8\height}{ \rotatebox[origin=]{90}{Proposed-l0}}
%   \begin{subfigure}{2.0in}
%  \begin{tikzpicture}
%    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=2.0in,height=2.0in,keepaspectratio]{sec/images/proposedlo_data2.png}};
%     \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[red,ultra thick,sharp corners] (0.07,0.65) rectangle (0.13,0.57);
%     \end{scope}
%      \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[blue,ultra thick,sharp corners] (0.35,0.57) rectangle (0.39,0.53);
%     \end{scope}
% \end{tikzpicture}
%  \caption{PSNR = 24.87, SSIM = 0.88}}
%   \end{subfigure}\hfill
%   \begin{subfigure}{2.0in}
% \adjustbox{cfbox=red 1pt}{\includegraphics[width=2cm,trim={95 420 1125 266},clip,width=2.0in,height=2.0in,keepaspectratio]{sec/images/proposedlo_data2.png}}
%   \end{subfigure}\hfill
%   \begin{subfigure}{2.0in}
% \adjustbox{cfbox=blue 1pt}{\includegraphics[width=2cm,trim={ 450 380 780 311},clip,width=2.0in,height=2.0in,keepaspectratio]{sec/images/proposedlo_data2.png}}  \end{subfigure}\hfill\\
% \raisebox{.8\height}{ \rotatebox[origin=]{90}{chen et al.\cite{chen2021learning}  }}
%  \begin{subfigure}{2.0in}
%  \begin{tikzpicture}
%    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=2.0in,height=2.0in,keepaspectratio]{sec/images/learning_data2.png}};
%     \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[red,ultra thick,sharp corners] (0.035,0.65) rectangle (0.095,0.57);
%     \end{scope}
%      \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[blue,ultra thick,sharp corners] (0.35,0.57) rectangle (0.39,0.53);
%     \end{scope}
% \end{tikzpicture}
%  \caption{PSNR = 19.20, SSIM = 0.74}}
%   \end{subfigure}\hfill
%   \begin{subfigure}{2.0in}
% \adjustbox{cfbox=red 1pt}{\includegraphics[width=2cm,trim={30 320 885 195},clip,width=2.0in,height=2.0in,keepaspectratio]{sec/images/learning_data2.png}}
%   \end{subfigure}\hfill
%   \begin{subfigure}{2.0in}
% \adjustbox{cfbox=blue 1pt}{\includegraphics[width=2cm,trim={ 321 287 595 228},clip,width=2.0in,height=2.0in,keepaspectratio]{sec/images/learning_data2.png}}
% \end{subfigure}\hfill\\

% \raisebox{.8\height}{ \rotatebox[origin=]{90}{Pan et al. \cite{pan2016blind}}}
%  \begin{subfigure}{2.0in}
%  \begin{tikzpicture}
%    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=2.0in,height=2.0in,keepaspectratio]{sec/images/cvpr16_data2.png}};
%     \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[red,ultra thick,sharp corners] (0.07,0.65) rectangle (0.13,0.57);
%     \end{scope}
%      \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[blue,ultra thick,sharp corners] (0.35,0.57) rectangle (0.39,0.53);
%     \end{scope}
% \end{tikzpicture}
%  \caption{PSNR = 22.07, SSIM = 0.77}}
%   \end{subfigure}\hfill
%   \begin{subfigure}{2.0in}
% \adjustbox{cfbox=red 1pt}{\includegraphics[width=2cm,trim={92 420 1128 266},clip,width=2.0in,height=2.0in,keepaspectratio]{sec/images/cvpr16_data2.png}}
%   \end{subfigure}\hfill
%   \begin{subfigure}{2.0in}
% \adjustbox{cfbox=blue 1pt}{\includegraphics[width=2cm,trim={ 449 380 781 311},clip,width=2.0in,height=2.0in,keepaspectratio]{sec/images/cvpr16_data2.png}}
% \end{subfigure}\hfill\\

% \vspace{0.0in}
% \raisebox{.8\height}{ \rotatebox[origin=]{90}{Chen et al. \cite{chen2020oid} }}  
%   \begin{subfigure}{2.0in}
%  \begin{tikzpicture}
%    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=2.0in,height=2.0in,keepaspectratio]{sec/images/outliner_data2.png}};
%     \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[red,ultra thick,sharp corners] (0.07,0.65) rectangle (0.13,0.57);
%     \end{scope}
%      \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[blue,ultra thick,sharp corners] (0.35,0.57) rectangle (0.39,0.53);
%     \end{scope}
% \end{tikzpicture}
%  \caption{PSNR = 22.22, SSIM = 0.76}
%   \end{subfigure}\hfill
% \begin{subfigure}{2.0in}
% \adjustbox{cfbox=red 1pt}{\includegraphics[width=2cm,trim={92 420 1128 267},clip,width=2.0in,height=2.0in,keepaspectratio]{sec/images/outliner_data2.png}}
% \end{subfigure}\hfill
% \begin{subfigure}{2.0in}
% \adjustbox{cfbox=blue 1pt}{\includegraphics[width=2cm,trim={ 449 380 781 312},clip,width=2.0in,height=2.0in,keepaspectratio]{sec/images/outliner_data2.png}}  \end{subfigure}\hfill\\
% \raisebox{.8\height}{ \rotatebox[origin=]{90}{Chen et. al\cite{chen2021blind} }}
%     \begin{subfigure}{2.0in}
%  \begin{tikzpicture}
%    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=2.0in,height=2.0in,keepaspectratio]{sec/images/saturate_data2.png}};
%     \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[red,ultra thick,sharp corners] (0.07,0.65) rectangle (0.13,0.57);
%     \end{scope}
%      \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[blue,ultra thick,sharp corners] (0.35,0.57) rectangle (0.39,0.53);
%     \end{scope}
% \end{tikzpicture}
%  \caption{PSNR = 24.17, SSIM = 0.86}
%   \end{subfigure}\hfill
% \begin{subfigure}{2.0in}
% \adjustbox{cfbox=red 1pt}{\includegraphics[width=2cm,trim={92 420 1129 268},clip,width=2.0in,height=2.0in,keepaspectratio]{sec/images/saturate_data2.png}}
% \end{subfigure}\hfill
% \begin{subfigure}{2.0in}
% \adjustbox{cfbox=blue 1pt}{\includegraphics[width=2cm,trim={ 448 380 782 312},clip,width=2.0in,height=2.0in,keepaspectratio]{sec/images/saturate_data2.png}}  \end{subfigure}\hfill\\

% \raisebox{.8\height}{ \rotatebox[origin=]{90}{Hu et al. \cite{hu2014deblurring} }}
%     \begin{subfigure}{2.0in}
%  \begin{tikzpicture}
%    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=2.0in,height=2.0in,keepaspectratio]{sec/images/streak_data2.png}};
%     \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[red,ultra thick,sharp corners] (0.07,0.65) rectangle (0.13,0.57);
%     \end{scope}
%      \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[blue,ultra thick,sharp corners] (0.35,0.57) rectangle (0.39,0.53);
%     \end{scope}
% \end{tikzpicture}
%    \caption{PSNR = 15.04, SSIM = 0.64}
%   \end{subfigure}\hfill
% \begin{subfigure}{2.0in}
% \adjustbox{cfbox=red 1pt}{\includegraphics[width=2cm,trim={93 419 1129 268},clip,width=2.0in,height=2.0in,keepaspectratio]{sec/images/streak_data2.png}}
% \end{subfigure}\hfill
% \begin{subfigure}{2.0in}
% \adjustbox{cfbox=blue 1pt}{\includegraphics[width=2cm,trim={ 450 380 780 311},clip,width=2.0in,height=2.0in,keepaspectratio]{sec/images/streak_data2.png}}  \end{subfigure}\hfill\\
\label{real_dataset}
% \caption{Comparison of the proposed framework, including \cite{xu2010two} and\cite{wen2020simple} and as deblurring methods, with the sate of the art SADT. The PSNR and SSIM are presented for the entire dataset whereas, for visual comparision on reprevtative image is randonly selected from the dataset % 
% \end{figure*}
In Figure \ref{varying_blur} and Table \ref{varying_blur_metrics}, we perform the quantative assessment of the propsed methods with the wide range of both saturation aware as well as more genral purpose image deblurring technique to esure the inclusivity of the most recent advancment in image resotrion, speficlay we included the deep leraning based state of the art method in out comparsions. To fruther evlaute the robustness of the proposed methods we varied the amount of blur in the testing dataset \cite{hanji2021hdr4cv} by increasing the number consective frames mergerd from 2 to 5. In Figure \ref{varying_blur} it is evident that proposed method has an overall better performance than the diverse range seleted methods. However it should be noted that the (Structural Similarity Index) SSIM favors the proposed method siginfcalty than the 2nd best peroforming method where the gap in performance is sequed in Peak Signal-to-Noise Ratio (PSNR) comparison.  
\begin{figure}[!h]
\centering
{\includegraphics[trim={45 7 30 23},clip,width=3.5in,height=3.5in,keepaspectratio]{sec/images/Varying blur_result.pdf}}
 \label{varying_blur}
 \caption{COmparsion of the state of the art, saturation aware and general puropose deblurrying methods  with the propsed technique on a dataset with varying level of blur. A rondmly selected sample image from the blur dataset in presented in Figure \ref{blur_view}.}
\end{figure}
\begin{figure}[!h]
\centering
\begin{subfigure}{1.5in}
{\includegraphics[width=1.5in,height=1.5in,keepaspectratio]{sec/images/Blur_2.png}}
 \caption{Im \times 2}
\end{subfigure}
\begin{subfigure}{1.5in}
{\includegraphics[width=1.5in,height=1.5in,keepaspectratio]{sec/images/Blur_3.png}}
 \caption{Im \times 3}
\end{subfigure}\\
\begin{subfigure}{1.5in}
{\includegraphics[width=1.5in,height=1.5in,keepaspectratio]{sec/images/Blur_4.png}}
 \caption{Im \times 4}
\end{subfigure}
\begin{subfigure}{1.5in}
{\includegraphics[width=1.5in,height=1.5in,keepaspectratio]{sec/images/Blur_5.png}}
 \caption{Im \times 5}
\end{subfigure}\\
 \caption{SA represntative image of varying blur level from the data-set used to produces resutls in Figure \ref{varying_blur}. }
 \label{blur_view}
 \end{figure}
While SSIM  measures perceived changes in structural information, and PSNR quantifies the difference in pixel intensities, by weighting PSNR with SSIM, SSIM-Weighted PSNR emphasizes scenarios where perceptual quality is as important as signal fidelity.\cite{wang2010information}. 
 \[
   \text{SSIM-Weighted PSNR} = \text{PSNR} \times \text{SSIM}
   \]
Similarly, Normalized Product Quality (NPQ) combines normalized PSNR and SSIM scores by their geometric mean, thereby reducing the influence of one high value from skewing the result.
     \[
   \text{NPQ} = \sqrt{\left(\frac{\text{PSNR}}{\text{PSNR}_{\max}}\right) \cdot \left(\frac{\text{SSIM}}{\text{SSIM}_{\max}}\right)}
   \]

These metrics collectively provide a balanced view of image restoration, highlighting both signal fidelity and perceptual quality across methods, as preesented in Table \ref{varying_blur_metrics}.The proposed method demonstrate a whloestic superior performce in comparsion to both satutatition specific and more gneneral purpose learning and non-learning based deblurring methods.
\begin{table*}[]
\begin{tabular}{llllllllllllll}
\hline
\multicolumn{1}{|l|}{\multirow{}{}{Method}} & \multicolumn{1}{l|}{\multirow{}{}{Saturation handling}} & \multicolumn{6}{l|}{Normalized Product Quality}                                                                                                & \multicolumn{6}{l|}{SSIM-Weighted PSNR}                                                                                                        \\ \cline{3-14} 
\multicolumn{1}{|l|}{}                        & \multicolumn{1}{l|}{}                                     & \multicolumn{1}{c|}{Im2}   & \multicolumn{1}{c|}{Im3}   & \multicolumn{1}{c|}{Im4}   & \multicolumn{2}{c|}{Im5}   & \multicolumn{1}{c|}{Avg.}  & \multicolumn{1}{c|}{Im2}   & \multicolumn{1}{c|}{Im3}   & \multicolumn{1}{c|}{Im4}   & \multicolumn{2}{c|}{Im5}   & \multicolumn{1}{l|}{Avg.}  \\ \hline
\multicolumn{1}{|l|}{Proposed}                & \multicolumn{1}{l|}{Saturation Handling}                  & \multicolumn{1}{l|}{0.955} & \multicolumn{1}{l|}{0.960} & \multicolumn{1}{l|}{0.945} & \multicolumn{2}{l|}{0.920} & \multicolumn{1}{l|}{0.945} & \multicolumn{1}{l|}{28.38} & \multicolumn{1}{l|}{28.49} & \multicolumn{1}{l|}{27.11} & \multicolumn{2}{l|}{25.63} & \multicolumn{1}{l|}{27.40} \\ \hline
\multicolumn{1}{|l|}{chen{[}10{]}}            & \multicolumn{1}{l|}{Saturation Handling}                  & \multicolumn{1}{l|}{0.825} & \multicolumn{1}{l|}{0.785} & \multicolumn{1}{l|}{0.770} & \multicolumn{2}{l|}{0.740} & \multicolumn{1}{l|}{0.780} & \multicolumn{1}{l|}{25.77} & \multicolumn{1}{l|}{23.60} & \multicolumn{1}{l|}{22.17} & \multicolumn{2}{l|}{20.81} & \multicolumn{1}{l|}{13.60} \\ \hline
\multicolumn{1}{|l|}{Kong{[}16{]}}            & \multicolumn{1}{l|}{General}                              & \multicolumn{1}{l|}{0.870} & \multicolumn{1}{l|}{0.890} & \multicolumn{1}{l|}{0.850} & \multicolumn{2}{l|}{0.820} & \multicolumn{1}{l|}{0.857} & \multicolumn{1}{l|}{26.83} & \multicolumn{1}{l|}{27.36} & \multicolumn{1}{l|}{25.70} & \multicolumn{2}{l|}{23.80} & \multicolumn{1}{l|}{14.89} \\ \hline
\multicolumn{1}{|l|}{Wang{[}9{]}}             & \multicolumn{1}{l|}{Night}                                & \multicolumn{1}{l|}{0.875} & \multicolumn{1}{l|}{0.860} & \multicolumn{1}{l|}{0.820} & \multicolumn{2}{l|}{0.790} & \multicolumn{1}{l|}{0.836} & \multicolumn{1}{l|}{26.85} & \multicolumn{1}{l|}{26.00} & \multicolumn{1}{l|}{24.01} & \multicolumn{2}{l|}{22.61} & \multicolumn{1}{l|}{14.31} \\ \hline
\multicolumn{1}{|l|}{Laroche{[}8{]}}          & \multicolumn{1}{l|}{Saturation Handling}                  & \multicolumn{1}{l|}{0.880} & \multicolumn{1}{l|}{0.870} & \multicolumn{1}{l|}{0.840} & \multicolumn{2}{l|}{0.810} & \multicolumn{1}{l|}{0.850} & \multicolumn{1}{l|}{26.87} & \multicolumn{1}{l|}{26.46} & \multicolumn{1}{l|}{24.36} & \multicolumn{2}{l|}{22.66} & \multicolumn{1}{l|}{14.53} \\ \hline
\multicolumn{1}{|l|}{Zamir{[}7{]}}            & \multicolumn{1}{l|}{General}                              & \multicolumn{1}{l|}{0.925} & \multicolumn{1}{l|}{0.930} & \multicolumn{1}{l|}{0.900} & \multicolumn{2}{l|}{0.860} & \multicolumn{1}{l|}{0.904} & \multicolumn{1}{l|}{27.76} & \multicolumn{1}{l|}{27.89} & \multicolumn{1}{l|}{25.93} & \multicolumn{2}{l|}{23.85} & \multicolumn{1}{l|}{15.13} \\ \hline
\multicolumn{1}{|l|}{Hu{[}15{]}}              & \multicolumn{1}{l|}{Saturation Handling}                  & \multicolumn{1}{l|}{0.685} & \multicolumn{1}{l|}{0.690} & \multicolumn{1}{l|}{0.700} & \multicolumn{2}{l|}{0.705} & \multicolumn{1}{l|}{0.695} & \multicolumn{1}{l|}{17.99} & \multicolumn{1}{l|}{19.40} & \multicolumn{1}{l|}{19.87} & \multicolumn{2}{l|}{19.94} & \multicolumn{1}{l|}{12.36} \\ \hline
\multicolumn{1}{|l|}{Jinshan{[}11{]}}         & \multicolumn{1}{l|}{Night}                                & \multicolumn{1}{l|}{0.775} & \multicolumn{1}{l|}{0.780} & \multicolumn{1}{l|}{0.755} & \multicolumn{2}{l|}{0.750} & \multicolumn{1}{l|}{0.765} & \multicolumn{1}{l|}{22.36} & \multicolumn{1}{l|}{22.66} & \multicolumn{1}{l|}{22.12} & \multicolumn{2}{l|}{21.44} & \multicolumn{1}{l|}{14.00} \\ \hline
\multicolumn{1}{|l|}{Liang{[}13{]}}           & \multicolumn{1}{l|}{Saturation Handling}                  & \multicolumn{1}{l|}{0.790} & \multicolumn{1}{l|}{0.785} & \multicolumn{1}{l|}{0.760} & \multicolumn{2}{l|}{0.740} & \multicolumn{1}{l|}{0.769} & \multicolumn{1}{l|}{22.82} & \multicolumn{1}{l|}{22.63} & \multicolumn{1}{l|}{21.62} & \multicolumn{2}{l|}{20.73} & \multicolumn{1}{l|}{13.66} \\ \hline
\multicolumn{1}{|l|}{Liang{[}12{]}}           & \multicolumn{1}{l|}{Saturation Handling}                  & \multicolumn{1}{l|}{0.655} & \multicolumn{1}{l|}{0.645} & \multicolumn{1}{l|}{0.630} & \multicolumn{2}{l|}{0.620} & \multicolumn{1}{l|}{0.638} & \multicolumn{1}{l|}{18.33} & \multicolumn{1}{l|}{18.00} & \multicolumn{1}{l|}{17.18} & \multicolumn{2}{l|}{16.16} & \multicolumn{1}{l|}{11.67} \\ \hline
\multicolumn{1}{|l|}{Alam{[}3{]}}             & \multicolumn{1}{l|}{General}                              & \multicolumn{1}{l|}{0.705} & \multicolumn{1}{l|}{0.710} & \multicolumn{1}{l|}{0.680} & \multicolumn{2}{l|}{0.670} & \multicolumn{1}{l|}{0.69}  & \multicolumn{1}{l|}{19.96} & \multicolumn{1}{l|}{19.62} & \multicolumn{1}{l|}{18.54} & \multicolumn{2}{l|}{17.60} & \multicolumn{1}{l|}{12.44} \\ \hline
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                            \\
                                              &                                                           &                            &                            &                            &              &             &                            &                            &                            &                            &              &             &                           
\end{tabular}
\label{varying_blur_metrics}
\end{table*}

In Figure \ref{building} we qualatitevly test our proposed framwork on a real blurry image from \cite{lai2016comparative} with relatively smaller region effected by the blur. We demosntrate that saturion effecting even a fever pixels can degragred the perofmrance of image resotration techniques. To produce the results in this figure, we followed \cite{shu2024deep}, in  estimating the blur kernel using  \cite{pan2016robust}.  While \cite{chen2021blind} couldn't completly revocwer from the blur \cite{chen2021learning,zhang2017learning}, introduced additional rinign artificats. \cite{shu2024deep} restore the information lost due blur in certian region but is the only method the does not  reduce signifcant blur as visible in the bar lines and text in the zoomed in region, thus avoids the deburring artifcats, visible in\cite{chen2021learning,zhang2017learning}.   The propsed method however, siginficantly reduce the blur without introduicng any additional ringing artifcats.

\begin{figure*}[!h]
\centering
\begin{subfigure}{1.1in}
{\includegraphics[width=1.1in,height=1.1in,keepaspectratio]{sec/images/Input.png}}
 \caption{Input}
\end{subfigure}\hfill
\begin{subfigure}{1.1in}
{\includegraphics[width=1.1in,height=1.1in,keepaspectratio]{sec/images/chen.png}}
 \caption{chen et al.\cite{chen2021blind}}
\end{subfigure}\hfill
\begin{subfigure}{1.1in}
{\includegraphics[width=1.1in,height=1.1in,keepaspectratio]{sec/images/ircnn.png}}
 \caption{Zhang et al. \cite{zhang2017learning}}
\end{subfigure}\hfill
\begin{subfigure}{1.1in}
{\includegraphics[width=1.1in,height=1.1in,keepaspectratio]{sec/images/nbdn.png}}
 \caption{chen et al. \cite{chen2021learning}}
\end{subfigure}\hfill
\begin{subfigure}{1.1in}
{\includegraphics[width=1.1in,height=1.1in,keepaspectratio]{sec/images/plugnplay.png}}
 \caption{Shu et al. \cite{shu2024deep}}
\end{subfigure}\hfill
\begin{subfigure}{1.1in}
{\includegraphics[width=1.1in,height=1.1in,keepaspectratio]{sec/images/Propbuilding.png}}
 \caption{Proposed}
\end{subfigure}\\
\label{building}
\caption{}
\end{figure*}
 We further, demonstrate in  Figure \ref{sat_effect} that the sucess of the  proposed framework is dervied for effectively handling the saturation in the image and any typical  SVBID method could benefit from it. We present two different images selected randomly from the publicaly availbe \cite{blur_dataset}  mobile phone data to visualy compare the deblurring results \cite{xu2010two} when included in the proposed saturated image deburring framework as a blind image deblurring method and direct application  of \cite{blur_dataset} .

\begin{figure*}[!h]
\centering
\begin{subfigure}{2.1in}
{\includegraphics[width=2.1in,height=2.1in,keepaspectratio]{sec/images/prop_cooler.png}}
 \caption{Input}
\end{subfigure}\hfill
\begin{subfigure}{2.1in}
{\includegraphics[width=2.1in,height=2.1in,keepaspectratio]{sec/images/xu_cooler.png}}
 \caption{chen et al.\cite{chen2021blind}}
\end{subfigure}\hfill
\begin{subfigure}{2.1in}
{\includegraphics[width=2.1in,height=2.1in,keepaspectratio]{sec/images/prop_bin.png}}
 \caption{Zhang et al. \cite{zhang2017learning}}
\end{subfigure}\hfill
\begin{subfigure}{2.1in}
{\includegraphics[width=2.1in,height=2.1in,keepaspectratio]{sec/images/xu_bin.png}}
 \caption{chen et al. \cite{chen2021learning}}
\end{subfigure}\hfill

\label{building}
\caption{}
\end{figure*}

% \begin{figure*}[!h]
% \centering
% % \begin{subfigure}{2.0in}
% % {\includegraphics[trim={85 40 230 68},clip,width=2.0in,height=2.0in,keepaspectratio]{sec/images/Real_result.pdf}}
% %  \caption{Seahorse}
% % \end{subfigure}\\
%  \begin{subfigure}{2.0in}
%  \begin{tikzpicture}
%    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=2.0in,height=2.0in,keepaspectratio]{sec/images/propbin.jpg}};
%     \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[red,ultra thick,sharp corners] (0.78,0.83) rectangle (0.88,0.92);
%     \end{scope}
%      \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[blue,ultra thick,sharp corners] (0.40,0.85) rectangle (0.50,0.94);
%     \end{scope}
% \end{tikzpicture}
% \end{subfigure}\\
%   \hspace{-0.07in}
%   \begin{subfigure}{0.96in}
%   \setlength{\fboxsep}{0pt}
% \adjustbox{cfbox=blue 1pt}{\includegraphics[trim={420 573 521 48},clip,width=0.96in,height=0.96in,keepaspectratio]{sec/images/propbin.jpg}}
%   \end{subfigure}
%   \begin{subfigure}{0.975in}
%   \setlength{\fboxsep}{0pt}
% \adjustbox{cfbox=red 1pt}{\includegraphics[trim={ 810 573 131 49},clip,width=0.975in,height=0.975in,keepaspectratio]{sec/images/propbin.jpg}}  \end{subfigure}\\
%  \begin{subfigure}{2.0in}
%  \begin{tikzpicture}
%    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=2.0in,height=2.0in,keepaspectratio]{sec/images/xubin.jpg}};
%     \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[red,ultra thick,sharp corners] (0.78,0.83) rectangle (0.88,0.92);
%     \end{scope}
%      \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[blue,ultra thick,sharp corners] (0.40,0.85) rectangle (0.50,0.94);
%     \end{scope}
% \end{tikzpicture}
% \end{subfigure}\\
%   \hspace{-0.07in}
%   \begin{subfigure}{0.96in}
%   \setlength{\fboxsep}{0pt}
% \adjustbox{cfbox=blue 1pt}{\includegraphics[trim={420 573 521 48},clip,width=0.96in,height=0.96in,keepaspectratio]{sec/images/xubin.jpg}}
%   \end{subfigure}
%   \begin{subfigure}{0.975in}
%   \setlength{\fboxsep}{0pt}
% \adjustbox{cfbox=red 1pt}{\includegraphics[trim={ 810 573 131 49},clip,width=0.975in,height=0.975in,keepaspectratio]{sec/images/xubin.jpg}}  \end{subfigure}\\
%  \begin{subfigure}{2.0in}
%  \begin{tikzpicture}
%    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=2.0in,height=2.0in,keepaspectratio]{sec/images/propcooler.jpg}};
%     \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[red,ultra thick,sharp corners] (0.19,0.40) rectangle (0.29,0.49);
%     \end{scope}
%      \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[blue,ultra thick,sharp corners] (0.40,0.85) rectangle (0.50,0.94);
%     \end{scope}
% \end{tikzpicture}
% \end{subfigure}\\
%   \hspace{-0.07in}
%   \begin{subfigure}{0.96in}
%   \setlength{\fboxsep}{0pt}
% \adjustbox{cfbox=red 1pt}{\includegraphics[trim={205 279 725 334},clip,width=0.96in,height=0.96in,keepaspectratio]{sec/images/propcooler.jpg}}
%   \end{subfigure}
%   \begin{subfigure}{0.975in}
%   \setlength{\fboxsep}{0pt}
% \adjustbox{cfbox=blue 1pt}{\includegraphics[trim={ 420 573 521 49},clip,width=0.975in,height=0.975in,keepaspectratio]{sec/images/propcooler.jpg}}  \end{subfigure}\\
%  \begin{subfigure}{2.0in}
%  \begin{tikzpicture}
%    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=2.0in,height=2.0in,keepaspectratio]{sec/images/xucooler.jpg}};
%     \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[red,ultra thick,sharp corners] (0.19,0.40) rectangle (0.29,0.49);
%     \end{scope}
%      \begin{scope}[x={(image.south east)},y={(image.north west)}]
%         \draw[blue,ultra thick,sharp corners] (0.40,0.85) rectangle (0.50,0.94);
%     \end{scope}
% \end{tikzpicture}
% \end{subfigure}\\
%   \hspace{-0.07in}
%   \begin{subfigure}{0.96in}
%   \setlength{\fboxsep}{0pt}
% \adjustbox{cfbox=red 1pt}{\includegraphics[trim={205 279 725 334},clip,width=0.96in,height=0.96in,keepaspectratio]{sec/images/xucooler.jpg}}
%   \end{subfigure}
%   \begin{subfigure}{0.975in}
%   \setlength{\fboxsep}{0pt}
% \adjustbox{cfbox=blue 1pt}{\includegraphics[trim={ 420 573 521 49},clip,width=0.975in,height=0.975in,keepaspectratio]{sec/images/xucooler.jpg}}  \end{subfigure}\\
%  \label{sat_effect}
%  \end{figure*}








% \setlength{\fboxsep}{0pt}
% \begin{subfigure}{2.0in}
% \adjustbox{cfbox=green 2pt}{\includegraphics[width=2cm,trim={ 630 616 295 10},clip,width=2.0in,height=2.0in,keepaspectratio]{sec/images/prop.jpg}}  \end{subfigure}\hfill\\
 



